VITAL: More Understandable Feature Visualization through Distribution Alignment and Relevant Information Flow

Neural networks are widely adopted to solve complex and challenging tasks. Especially in high-stakes decision-making, understanding their reasoning process is crucial, yet proves challenging for modern deep networks. Feature visualization (FV) is a powerful tool to decode what information neurons are responding to and hence to better understand the reasoning behind such networks. In particular, in FV we generate human-understandable images that reflect the information detected by neurons of interest. However, current methods often yield unrecognizable visualizations, exhibiting repetitive patterns and visual artifacts that are hard to understand for a human. To address these problems, we propose to guide FV through statistics of real image features combined with measures of relevant network flow to generate prototypical images. Our approach yields human-understandable visualizations that both qualitatively and quantitatively improve over state-of-the-art FVs across various architectures. As such, it can be used to decode which information the network uses, complementing mechanistic circuits that identify where it is encoded. Code is available at: https://github.com/adagorgun/VITAL

==> fig/fig_ablation_layer.tex <==



\begin{figure}
    \centering
    \centerline{\includegraphics[width=\linewidth]
    {fig/ablation_effect_layer.png}}
    \caption{}
    \label{fig:fig_ablation_layer}

\end{figure}

==> fig/fig_abstract.tex <==



\begin{figure}
    \centering
    \centerline{\includegraphics[width=\linewidth]
    {fig/abstract.png}}
    \caption{\textit{Feature visualization through distribution
alignment.} Existing work on feature visualization reveals which aspects of the data neural network components respond to, yet often yield unrecognizable, repetitive patterns
    that are uninformative to a user. We suggest a new paradigm, \ours, based on matching feature distributions of real images and taking into account feature relevance (\textcolor{arrow_color}{arrows}), that yields more understandable feature visualizations.}
    
    % \bernt{a few comments: (1) is the second example convincing to you - it is not to me actually, (2) scalability to ResNet is unclear if that is a challenge - there are quite shallow ResNets  actually - so `scaling' to ResNet per se it NOT compelling (3) here the term `recognizable' is used - but the title makes the point about more `understandable' - can we use the term `understandable' here as well? otherwise the teaser-figure seems not to fully support the story really as far as i am concerned (4) the list of `issues' is referring to existing efforts - but for the right side (e.g. `no repetition') it is not crystal clear that it refers to `VITAL (ours)' - this needs fine-tuning imho to leave no room for ambiguous interpretation}}
    \label{fig:fig_abstract}

\end{figure}

==> fig/fig_diversity.tex <==



\begin{figure}
    \centering
    \centerline{\includegraphics[width=.7\linewidth]
    {fig/diversity.png}}
    \caption{\textbf{Disentangling polysemanticity.} Existing FV methods can generate visualizations that strongly activate for unrelated concepts. In this example, given channel \#1660, \textbf{(first column)} a MACO visualization activates both on \textbf{(second column)} "digital clock" and "cauliflower". With VITAL, \textbf{(third column)} we can disentangle these concepts as separate visualizations. }
    \label{fig:fig_diversity}

\end{figure}




==> fig/fig_method_sm_app.tex <==



\begin{figure*}
    \centering
    \centerline{\includegraphics[width=\linewidth]
    {fig/method_sm_app.png}}
    \caption{\textbf{Overview of VITAL framework.} Our \ours framework consists of \bernt{the figure is huge - I doubt we will have the space for such a large figure}}
    \label{fig:fig_method_sm_app}

\end{figure*}



==> fig/fig_transparency.tex <==



\begin{figure}
    \centering
    \centerline{\includegraphics[width=\linewidth]
    {fig/transparency.png}}
    \caption{}
    \label{fig:fig_transparency}

\end{figure}

==> fig/rebuttal_corrupt.tex <==
\begin{wrapfigure}{r}{0.21\textwidth} % 'r' for right, 'l' for left
    % \centering
    \renewcommand{\figurename}{Fig.} % Local change
    \setlength{\abovecaptionskip}{5pt}
    \vspace{-10pt} % optional: tweak spacing
    \includegraphics[width=\linewidth]{fig/corrupt.png}
    \caption{Corruption}
    \vspace{-20pt} % optional: tweak spacing
    \label{fig:fig_rebuttal_corrupt}
\end{wrapfigure}

==> fig/rebuttal_fig.tex <==
\begin{figure}
\renewcommand{\figurename}{Fig.} % Local change
    \setlength{\abovecaptionskip}{5pt}
    \centering
    \includegraphics[width=.7\linewidth]{fig/visualizations_clusters.png}    
    \caption{$\blacksquare$: VITAL, $\blacktriangle $: cluster center}
    \label{fig:rebuttal_cluster}
    \vspace{-10pt}
\end{figure}




==> fig/rebuttal_whole.tex <==
\begin{figure}
\renewcommand{\figurename}{Fig.} % Local change
    \setlength{\abovecaptionskip}{5pt}
    \centering
    \begin{subfigure}{0.44\linewidth}
        \centering
        \raisebox{1mm}{\includegraphics[width=\linewidth]{fig/corrupt.png}}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.55\linewidth}
        \centering
        \raisebox{2mm}{\includegraphics[width=\linewidth]{fig/visualizations_clusters.png}}
    \end{subfigure}
    
    \caption{(left) Corruption, (right) $\blacksquare$: VITAL, $\blacktriangle $: cluster center}
    \label{fig:rebuttal_whole}
    % \vspace{-20pt}
\end{figure}




==> table/rebuttal_table.tex <==
% \begin{wraptable}{r}{0.28\textwidth}
%     \renewcommand{\tablename}{Tab.} % Local change
%     \setlength{\abovecaptionskip}{5pt}
%     \vspace{-10pt} % adjust to shift table upwards
%     \centering
%     \tiny
%     \begin{tabular}{lcccc}
%         \toprule
%         & \multicolumn{1}{c}{Acc.} & FID & \multicolumn{2}{c}{Zero-Shot Pred.} \\
%         \cmidrule(lr){4-5}
%         & Top1 $\uparrow$ & $\downarrow$ & Top1 $\uparrow$& Top5 $\uparrow$\\
%         \midrule
%         \textbf{Test Set} & 99.27 & 65.93 & 61.63 &89.30  \\
%         Train Set & 99.90 & 58.79 & 66.62 & 92.56 \\
%         Corrupt-5 & 99.97 & 72.73 & 61.03 & 88.80 \\
%         Corrupt-10 & 99.83 & 86.73 & 56.20 & 85.50 \\
%         Corrupt-20 & 99.93 & 113.30 & 47.30 & 77.40 \\
%         \midrule
%         \textbf{CIFAR-10} & - & - & 85.47 & 99.09 \\
%         VITAL &  &  & 90.00 & 100.00 \\
%         % \bottomrule
%     \end{tabular}
%     % \caption{Results}
%     \label{tab:rebuttal}
%     \vspace{-20pt} % adjust to reduce space below table
% \end{wraptable}

\begin{table}[]
    \renewcommand{\tablename}{Tab.} % Local change
    \setlength{\abovecaptionskip}{2pt}
    % \vspace{-10pt} % adjust to shift table upwards
    \centering
    \scriptsize
    \begin{tabular}{lcccc}
        \toprule
        & \multicolumn{1}{c}{Acc.} & FID & \multicolumn{2}{c}{Zero-Shot Prediction} \\
        \cmidrule(lr){4-5}
        & Top1 ($\uparrow$) & ($\downarrow$) & Top1 ($\uparrow$)& Top5 ($\uparrow$)\\
        \midrule
        \textbf{Test Set} & 99.27 & 65.93 & 61.63 &89.30  \\
        Train Set & 99.90 & 58.79 & 66.62 & 92.56 \\
        Corrupt-5 & 99.97 & 72.73 & 61.03 & 88.80 \\
        Corrupt-10 & 99.83 & 86.73 & 56.20 & 85.50 \\
        Corrupt-20 & 99.93 & 113.30 & 47.30 & 77.40 \\
        \midrule
        \textbf{CIFAR-10} & - & - & 85.47 & 99.09 \\
        Fourier & 5.97 & 34.87 & 11.40 & 53.80\\
        VITAL & 100.00 & 0.55 & 78.30 & 98.90\\
        
        % \bottomrule
    \end{tabular}
    \caption{Additional results}
    \label{tab:rebuttal}
    \vspace{-22pt} % adjust to reduce space below table
\end{table}

==> table/table_CLIP.tex <==


\begin{table}[]
    \centering
    \begin{tabular}{cccc}
        \toprule
         Images & Setup & Top-1 ($\uparrow$) & Top-5 ($\uparrow$) \\ 
         \midrule
         ImageNet & clean & 69.11 & 92.23 \\
         \hdashline\noalign{\vskip 1.0ex}
         \multirow{2}{*}{MACO \cite{Fel2023}} & res: 224 & 12.87 & 29.73 \\
          & res: 1024 & 1.60 & 5.67\\
          \hdashline\noalign{\vskip 1.0ex}
         \multirow{2}{*}{Fourier} & res: 224 & 6.73 & 18.27\\
          & res: 1024 & 0.97 & 3.57\\
          \hdashline\noalign{\vskip 1.0ex}
          \multirow{2}{*}{CBR} & res: 224 & 0.20 & 1.17\\
          & res: 1024 & 0.20 & 1.07\\
          \hdashline\noalign{\vskip 1.0ex}
         \multirow{2}{*}{DeepInv \cite{yin2020dreaming}}& batch size: 64 & 29.90 & 55.20 \\
          & batch size: 1 & 4.73 & 12.63\\
         \hdashline\noalign{\vskip 1.0ex}
         DeepInv \cite{yin2020dreaming}& batch size: 64 & 17.20 & 40.43 \\
         down ($\downarrow2$) & batch size: 1 & 6.30 & 16.43 \\
         \midrule
         \textbf{VITAL} & - & 66.62 & 92.56\\
         \bottomrule
         
    \end{tabular}
    \caption{Caption}
    \label{tab:CLIP}
\end{table}

==> table/table_FID.tex <==


\begin{table}[]
    \centering
    \begin{tabular}{cccc}
        \toprule
        Images & \multirow{2}{*}{Setup} & \multicolumn{2}{c}{Zero-Shot Prediction} & FID ($\downarrow$) \\ 
         
         & &Top-1 ($\uparrow$) & Top-5 ($\uparrow$) & \\ 
         \midrule
         ImageNet & clean & 69.11 & 92.23 \\
         \hdashline\noalign{\vskip 1.0ex}
         \multirow{2}{*}{MACO \cite{Fel2023}} & res: 224 & 12.87 & 29.73 \\
          & res: 1024 & 1.60 & 5.67\\
          \hdashline\noalign{\vskip 1.0ex}
         \multirow{2}{*}{Fourier} & res: 224 & 6.73 & 18.27\\
          & res: 1024 & 0.97 & 3.57\\
          \hdashline\noalign{\vskip 1.0ex}
          \multirow{2}{*}{CBR} & res: 224 & 0.20 & 1.17\\
          & res: 1024 & 0.20 & 1.07\\
          \hdashline\noalign{\vskip 1.0ex}
         \multirow{2}{*}{DeepInv \cite{yin2020dreaming}}& batch size: 64 & 29.90 & 55.20 \\
          & batch size: 1 & 4.73 & 12.63\\
         \hdashline\noalign{\vskip 1.0ex}
         DeepInv \cite{yin2020dreaming}& batch size: 64 & 17.20 & 40.43 \\
         down ($\downarrow2$) & batch size: 1 & 6.30 & 16.43 \\
         \midrule
         \textbf{VITAL} & - & 66.62 & 92.56\\
         \bottomrule
         
    \end{tabular}
    \caption{Caption}
    \label{tab:combined}
\end{table}

==> table/table_classification.tex <==


\begin{table}[t]
    \centering
    \footnotesize
    \begin{tabular}{cccccc}
        \toprule
         \multirow{2}{*}{Images} & \multicolumn{2}{c}{Tiger} & \multicolumn{2}{c}{Maltese dog}  \\ 
         \cmidrule{2-5}
         & \#1 score & \#2 score & \#1 score  & \#2 score \\
         \midrule
         \multirow{2}{*}{ImageNet} &  \textbf{Tiger} &  \textbf{Tiger cat} &  \textbf{Maltese dog} & \textbf{Lhasa} \\
         & 0.8625 &  0.1363 & 0.9757 & 0.0149\\
         \hdashline\noalign{\vskip 1.0ex}
         \multirow{2}{*}{MACO}  &  \textbf{Tiger} & \textbf{Apiary} & \textcolor{arrow_color}{\textbf{Silky terrier}} & \textbf{Coral reef} \\         
         & 0.5752 & 0.1616 & 0.4127 & 0.2002 \\
          \hdashline\noalign{\vskip 1.0ex}
         \multirow{2}{*}{DeepInv} & \textbf{Tiger} &  \textbf{Tiger cat} &  \textbf{Maltese dog} &  \textbf{Lhasa} \\
         & 0.9984 & 0.0013 & 0.9989 & 0.0004 \\
         \midrule
         \multirow{2}{*}{\textbf{VITAL}} & \textbf{Tiger} &  \textbf{Tiger cat} &  \textbf{Maltese dog} &  \textbf{Lhasa} \\
         & 0.8609 & 0.1382 & 0.9797 & 0.0112\\
         \bottomrule
         
    \end{tabular}
    \caption{Comparison of top-2 softmax scores of example classes across methods applied on ResNet50 trained on ImageNet. We use MACO with resolution 224 and DeepInv with batch size 64 (best setting in previous experiments) and indicate  \textcolor{arrow_color}{\textbf{misclassification}}. }
    \label{tab:accuracy}
\end{table}



==> table/table_combined.tex <==
\begin{table}[t]
    \centering
    \footnotesize
    \begin{tabular}{cccccc}
        \toprule
         \multirow{2}{*}{Method} & \multirow{2}{*}{Setup} &Acc. &  \multirow{2}{*}{FID ($\downarrow$)}& \multicolumn{2}{c}{Zero-Shot Prediction}   \\ 
         \cmidrule{5-6}%\cmidrule{6}
         & & Top1 ($\uparrow$) & & Top1 ($\uparrow$) & Top5 ($\uparrow$) \\
         \midrule
         ImageNet &  & - & -&  69.11 & 92.23 \\
         \hdashline\noalign{\vskip 1.0ex}
         \multirow{2}{*}{MACO} & r: 224 & 29.43 & 360.74 & 12.87 & 29.73 \\
         & r: 1024 & 2.10 & 494.57 & 1.60 & 5.67   \\
         \hdashline\noalign{\vskip 1.0ex}
         \multirow{2}{*}{Fourier} & r: 224 & 21.30 & 422.44 & 6.73 & 18.27  \\
         & r: 1024 & 3.43 & 430.58 & 0.97 & 3.57  \\
         \hdashline\noalign{\vskip 1.0ex}
         \multirow{2}{*}{CBR} & r: 224 & 0.50 & 545.50 & 0.20 & 1.17  \\
         & r: 1024 & 0.33 & 522.89 & 0.20 & 1.07  \\
         \hdashline\noalign{\vskip 1.0ex}
         \multirow{2}{*}{DeepInv}& bs: 64 & \textbf{100.00} & \textbf{35.76} & \textcolor{blue}{\textbf{29.90}} & \textcolor{blue}{\textbf{55.20}} \\
         & bs: 1 & \textbf{100.00} & 123.77 & 4.73 & 12.63  \\
         \hdashline\noalign{\vskip 1.0ex}
         DeepInv & bs: 64 & 50.47 & 176.35 & 17.20 & 40.43  \\
         ($\downarrow2$) & bs: 1 & \textbf{100.00} & 121.94 & 6.30 & 16.43  \\
         \midrule
         \textbf{VITAL} &  & \textcolor{blue}{\textbf{99.90}} & \textcolor{blue}{\textbf{58.79}} & \textbf{66.62} & \textbf{92.56}  \\
         \bottomrule
    \end{tabular}
    \caption{Comparison of methods on ResNet50 trained on Imagenet. We provide FID scores, CLIP Zero-shot prediction scores, and top-1 classification accuracy, indicating the \textbf{best} and \textcolor{blue}{\textbf{second best}}. In the settings, "r" indicates the resolution of the visualization and "bs" is the used batch size and indicate with ($\downarrow 2$) the multi-resolution optimization version of DeepInv.}
    \label{tab:combined}
\end{table}
